Speech Understanding on Tiny Devices with A Learning Cache

This paper addresses spoken language understanding (SLU) on microcontroller-like embedded devices, integrating on-device execution with cloud offloading in a novel fashion. We leverage temporal locality in the speech inputs to a device and reuse recent SLU inferences accordingly. Our idea is simple: let the device match incoming inputs against cached results, and only offload inputs not matched to any cached ones to the cloud for full inference. Realization of this idea, however, is non-trivial: the device needs to compare acoustic features in a robust yet low-cost way. To this end, we present SpeechCache (or SC), a speech cache for tiny devices. It matches speech inputs at two levels of representations: first by sequences of clustered raw sound units, then as sequences of phonemes. Working in tandem, the two representations offer complementary tradeoffs between cost and efficiency. To boost accuracy even further, our cache learns to personalize: with the mismatched and then offloaded inputs, it continuously finetunes the device's feature extractors with the assistance of the cloud. We implement SC on an off-the-shelf STM32 microcontroller. The complete implementation has a small memory footprint of 2MB. Evaluated on challenging speech benchmarks, our system resolves 45%-90% of inputs on device, reducing the average latency by up to 80% compared to offloading to popular cloud speech recognition services. The benefit brought by our proposed SC is notable even in adversarial settings - noisy environments, cold cache, or one device shared by a number of users.

==> conclusion.tex <==
\section{Conclusion}


==> fig-design-space.tex <==
% !TeX root = main.tex

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/design-space.pdf}
    \caption{The design space of speech understanding}
    \label{fig:design-space}
\end{figure}

==> fig-diff-opt.tex <==


\begin{table}[t]
\centering
\includegraphics[width=0.5\textwidth]{figs/diff-opt.pdf}
    % \includegraphics[width=0.5\textwidth]{figs/avg_latency_v_setting.png}
    \caption{Detailed evaluation of \sys{} on \slurp{} with different optimization combination shows that empirically selective bucketing and dynamic threshold gives the best performance in terms of accuracy.}
    
    \label{tab:do}
\end{table}


==> opt.tex <==
% !TeX root = main.tex

\section{Optimizations}

Split by lengths ...  multiple buckets...
[EXPERIMENT TO DO]

How to determine thresholds automatically....
[BY LENGTH/duration of input]






==> related.tex <==
% !TeX root = main.tex

\section{Related work}
\label{sec:related-work}

%\aben{discuss}
%\xzlNote{must cite RW's paper}
%
%\xzlNote{discuss ``learn to listen'' more carefully}

\paragraph{Spoken Language Understanding (SLU)} is discussed in \autoref{sec:slu}. 
%While a classic SLU pipeline runs multiple models in tandem, one for each pipeline stage, recent SLU pipelines often coalesce multiple stages (referred to as ``end-to-end'') \cite{serdyuk2018towards}, allowing joint optimization across the coalesced stages. For instance, one single model (multiple levels of transformers) can consume sound units and produce words (transcripts) or semantics. End to end SLU pipeline is promising as the need for intermediate steps is precluded. 
Existent SLU architectures employ convolutional \cite{mhiri2020low, tian2020improving} or recurrent \cite{palogiannidi2020end, liu2016joint, potdar2021streaming, lugosch2019speech} networks and perform compression to deploy on end device.



%SLU leverages a two-step pipeline: first an input speech is converted to text (ASR), then a language model (NLU) interprets the meaning behind a transcription. Although accurate, this pipeline can be compute expensive, error-prone and is non-personalized. Much has been done on fusing the ASR and NLU model in order to optimize the errors of a dual module pipeline \cite{radfar2021fans}.


%Automatic Speech Recognition (ASR) is a well-established/mature and extensively researched domain where spoken language is transcribed into text (STT) and the transcribed text is then further analyzed to recognize the intent (NLU). Although accurate, the pipeline can be compute expensive and error-prone. Much has been done on fusing the ASR and NLU model in order to optimize the errors of a dual module pipeline \cite{radfar2021fans}.
% With the advent of pretrained models such as wav2vec 2.0 \cite{baevski2020wav2vec}, the performance of speech recognition tasks has drastically improved, although they are computationally expensive. 


% Existent approach to process voice commands include two methods as explained in Lugosch et al \cite{lugosch2019speech}. In the conventional approach, there is a separate pipeline for speech recognition (ASR) and understanding the intent behind the text (NLU) \cite{borgholt2021we}. 
% % This involves converting speech to text and then analyzing the text to determine intent. 
% Conventional SLU does three tasks: domain classification, intent detection and slot filling. 

% \aben{moved from sec 2.2}


\begin{comment}
	can see related work of https://arxiv.org/pdf/2010.02295.pdf for SLU
	\cite{tian2020improving} cnn+repltile
	\cite{mhiri2020low} same authors from fluent, model size 1.3M but accuracy not better on fsc - cnn with segment pooling
	\cite{potdar2021streaming} - uses LSTM+CTC+CE, acc. on fsc and speech commands is like sota.
	\cite{myer2018efficient} - use cnn for kws (time delay nn)
	
\end{comment}

\paragraph{Keyword spotting (KWS)} is a sub problem of ASR \cite{vinyals2014chasing} and is defined as the task of identifying a predefined keyword (such as ``hey google``) in audio streams \cite{lopez2021deep}.
Voice assistants use KWS in order to be activated (``wake-up``) instead of running a computationally expensive ASR model \cite{vinyals2014chasing}. A small footprint KWS model does not scale well to large vocabularies and cannot perform well for longer commands. The reverse:  SLU capability on KWS tasks is verified by \cite{potdar2021streaming} - their E2E SLU model gives acceptable (if not better) accuracy on standard KWS tasks. 

%verify the capability of our model in spotting short key words?

%\paragraph{Keyword spotting}
%KWS is a subset of SLU (and simpler version of it), where a predefined voice command is used for waking up the device \cite{lopez2021deep}.
%Voice assistants deploy spoken keyword spotting(KWS) methodology in order to be activated instead of running a computationally expensive ASR model \cite{vinyals2014chasing}. Spoken KWS can be thought of as a sub problem of ASR \cite{vinyals2014chasing} and is defined as the task of identifying keywords in audio streams comprising speech \cite{lopez2021deep}. 
% Spoken language understanding (SLU) tasks are conventionally solved by transcribing an utterance using ASR and then feeding the output to a text-based model \cite{borgholt2021we}. 

 \paragraph{Query by Example (QbE)} is a template matching technique used for spoken term detection (STD) or KWS \cite{hazen2009query, lugosch2018donut}, the objective of which is to locate audio snippets containing keywords (enrollments) within a larger audio stream. But this technique is not well-suited for IC as the users need to explicitly define the "queries". 
% Hence for a device dictionary of 100 transcripts there needs to be 100 enrollments requiring $log(n^2)$ time complexity and significant memory. 
 Our feature extractor is significant since we can fine tune it (learnable) unlike QbE.
 
% Additionally there is no opportunity for learning/finetuning since it cannot be supervised by any large model. Our feature extractor is significant since we can fine tune it (learnable).


% \paragraph{Query by Example}
% \label{QbE}
% template matching qbe kws
% Query-by-Example (QbE) is a technique used for spoken term detection (STD) where the user provides a limited number (e.g one or three) of audio snippets (containing explicit keywords/queries) referred to as enrollment. The objective is to locate these enrollments within a larger audio stream. The process involves extracting features from the audio, calculating similarity between enrollment and segments of input stream using measures such as Dynamic Time Warping (DTW) or CTC (DONUT \cite{lugosch2018donut}) and identifying segments of the input audio that exhibit high similarity scores. \cite{hazen2009query} is one of the first to use phonetic posteriorgarams. for query by example spoken term detection. But this approach is not well-suited for our speech to intent classification task as the users need to explicitly define the "keywords" or "queries". Hence for a device dictionary of XX transcripts there needs to be XX enrollments requiring $log(n^2)$ time complexity. Additionally there is no opportunity for learning/finetuning since it cannot be supervised by any large model. Our feature extractor is significant since we can fine tune it (learnable)

% query by string - sample given in text form;worse than QbE since text might not match to voice

\textbf{Intent Classification (IC)} is discussed in \autoref{sec:slu}. 

%The task of understanding voice commands involves mapping the input audio signal to a structured format - intent (a three slot tuple) that can be comprehended by the device. 
%For a given voice command our goal is to simply categorize it into a specific intent category. 
IC is much more challenging (more words, requires contextual understanding) compared to KWS.

\cite{mun2020accelerating} uses a simple IC model based on string matching; \cite{myer2018efficient} uses a time delay NN architecture for KWS, caches intermediate results and skips frame to reduce compute. \cite{he2023can} incorporates prompting and in-context learning for IC using large pretrained language models. \cite{vacher2015speech} delineates the correlation between speech recognition performance and training size; an acceptable performance requires > 100 training data. As discussed in \autoref{sec:key-op}, our model is robust against this challenge. \cite{long2023ai} mentions exploring the opportunity to focus on short, complex commands with multiple elements instead of extended conversations. We dwell in the middle and focus on longer, complex but single intent commands. \cite{xu2020cha} introduces an intermediate caching framework (or hub) in between the edge and cloud for IC.
\cite{mcgraw2016personalized} employs a moderately small LSTM network large vocabulary speech recognition.
Multiple models employ content prefetching for service acceleration \cite{mun2020accelerating, schwarz2023personalized} . 
\cite{borgholt2021we} argues that learned speech features are superior to ASR transcripts on IC tasks - we exploit such rich learning opportunities in our model. \cite{arora2023universlu} shows that large language models does not necessarily perform better for IC and is an overkill.

Commercial off the shelf speech-to-intent engines such as rhino from PicoVoice \cite{picovoice_rhino}, Wio Terminal from Seeed studio \cite{WIO_terminal} etc. cannot scale to the performance of \sys{}. 

%Wio gives only 87.5\% accuracy on FSC, at 29kb (int8 quantization) and input has to be < 1s, costs \$42 .



%\textbf{Intent Classification:} In the context of information extraction Snips \cite{coucke2018snips} defines intent as something that corresponds to the action or intention contained in the user’s query, which can be more or less explicit. Such as for the voice command "Turn on the light", the intentName in Snips is \textit{switchLightOn}. The task of understanding voice commands involves mapping the input audio signal to an intent that the device can recognize. In the literature, intent, slot and entity has been interchangeably used as suited to the task at hand. For a given voice command our goal is to simply categorize it into a specific intent category.

% \cite{mun2020accelerating} uses a simple IC model based on string matching and does content prefetching for service acceleration. their IC model is too simple - string matching(BOW) - acc F1 - 60.36\%; reports cloud time - 1.11 (time), 1.64(weather), 4.88 (music), 8.54 (news), 12.19 (hue on). \cite{vacher2015speech} shows 'correlation between performance and training size' - 'users must record enough data before using the system' - for ambient assisted living.


%Intent classification is more intricate compared to keyword spotting (more words, contextual understanding) and models designed specifically for recognizing keywords may not be suitable for handling voice commands.



%\cite{sciutohey} shows how households incorporate voice assistants into their living
% perday, per-user median number of commands was 6.04.
% For households with three or four devices, it was 10.39,
% and for five and six it was 14.42.
% CHA, FSC, snips, hello-edge, donut

% (from wiki) Because the speech signal is not linear, there is a problem of segmentation. It is difficult to delimit a stretch of speech signal as belonging to a single perceptual unit. 

%aben: address later
% previous work doesnt address personalization/input complexity, resource constraints
% % \paragraph{speaker adaptation}

% % \paragraph{streaming}

% % \href{https://arxiv.org/pdf/2105.10042.pdf}{A Streaming End-to-End Framework For Spoken Language Understanding}
% \paragraph{why raw speech}
% "several studies have shown that deeplearning-based models with raw waveform inputs can achieve
% higher accuracy than those with hand-crafted features (e.g.,
% MFCC)"
% % Estimating
% % phoneme class conditional probabilities from raw speech
% % signal using convolutional neural networks,
% % Analysis of cnn-based speech
% % recognition system using raw speech as input,
% % "Very deep
% % convolutional neural networks for raw waveforms,
% % Raw Waveform-based Speech Enhancement by Fully
% % Convolutional Networks

%aben: address later
% LVCSR \cite{bahdanau2016end}, on smartphone\cite{lei2013accurate} \cite{mcgraw2016personalized}(LSTM with CTC, 20mb, rtf 0.14).
